Online Regularized Nonlinear Acceleration

Regularized nonlinear acceleration (RNA) estimates the minimum of a function by post-processing iterates from an algorithm such as the gradient method. It can be seen as a regularized version of Anderson acceleration, a classical acceleration scheme from numerical analysis. The new scheme provably improves the rate of convergence of fixed step gradient descent, and its empirical performance is comparable to that of quasi-Newton methods. However, RNA cannot accelerate faster multistep algorithms like Nesterov's method and often diverges in this context. Here, we adapt RNA to overcome these issues, so that our scheme can be used on fast algorithms such as gradient methods with momentum. We show optimal complexity bounds for quadratics and asymptotically optimal rates on general convex minimization problems. Moreover, this new scheme works online, i.e., extrapolated solution estimates can be reinjected at each iteration, significantly improving numerical performance over classical accelerated methods.

==> propositions/prop_asymptotic_optimal_rate.tex <==

    If $\tau = O(D^{-s})$ with $0<s<\alpha-1$, then, when $D\rightarrow 0$, Proposition \ref{prop:conv_nonlinear} becomes
    \BEAS
        & & \textstyle \left\|(G-I)(\yex-x^*)\right\| \\ 
        & \leq &  (1-\kappa)  \left(\frac{1-\sqrt{\kappa}}{1+\sqrt{\kappa}}\right)^{N-1}\left\|(G-I)(x_0-x^*)\right\|
    \EEAS
    The same result holds with Algorithm \ref{algo:rna} if $\lambda = O(D^r)$ with $0<r<2(\alpha-1)$.

==> sections/convergence_first_order_methods.tex <==

When we accelerate in particular the gradient descent algorithm, i.e.,
\[
    g(x) = x-h\nabla f(x),
\]
then we can write the results of Theorem \ref{thm:convergence_perturbation} more explicitely. Notice that our analysis also includes other gradient-step based algorithms, such as Nesterov's method, as they can be considered as a combination between a gradient step plus a momentum term. An extensive discusion on this topic can be found in Appendix \ref{sec:convergence_with_gd}, and we present here the main results. We will cover two different cases. The first one assumes each step of $g$ is corrupted by a random noise. The second case considers nonlinear updates $g(x)$ (for non quadratic minimization problems), and views them as a perturbation of the linear case (i.e., quadratic problems). 

\textbf{Optimizing quadratics with noisy gradients.} First, we consider the case where we optimize
\[
    f(x) = \frac{1}{2} (x-x^*)^TQ(x-x^*), \qquad \mu I \preceq Q \preceq LI.
\]
Of course, in practice the problem is not written under this form. However, this notation with $x^*$ makes the analysis simpler. Now, assume we use Algorithm \eqref{algo:cna} with \mbox{$\beta = 1$} on $N$ iterates from \eqref{eq:perturbed_iteration_matrix}, in the special case where the perturbation is an independent zero-mean noise with variance $\sigma^2$. In this case, Proposition \ref{prop:convergence_stoch_gradient} shows that
\[
    \textstyle \mathbb{E}[\|\nabla f(\yex)\|] \leq O(\cheb_{N-1}\|\nabla  f(x_0)\| + \frac{\sigma}{\sqrt{N}}).
\]
This means we have two different regimes. At the begining, when we are far from the optimum,  $\|\nabla  f(x_0)\| $ dominates $\sigma$. In this case, RNA enjoys an (near) optimal rate of convergence. Otherwise, when the noise dominates, the rate becomes similar to  averaged SGD.

\textbf{Optimizing nonquadratic functions.} In the special case where we use  gradient descent on non-quadratic functions, we have that
\[
    \tilde g(x) = x-h\nabla f(x) = \underbrace{x-h\nabla^2 f(x^*)(x-x^*)}_{=g(x)} + \underbrace{ h (\nabla^2 f(x^*)(x-x^*) - \nabla f(x))}_{=e_i}.
\]
Thus, the non-linear function $\tilde g$ can be reduced to a perturbed linear function $g(x)$ (eq. \eqref{eq:linear_g} with $G=I-h\nabla^2 f(x^*)$) with a nonlinear, nonrandom perturbation $e_i$. This setting can thus be analyzed using Theorem \ref{thm:convergence_perturbation}. Moreover, if we assume that $e_i$ is bounded such that
\[
    \|e_i\| \leq O(D^{\alpha}), \qquad  \text{where} \quad\|\tilde y_i-x^* \|_2 \leq D \;\;\forall i,
\]
then, when $D\rightarrow 0$, Proposition \ref{prop:asymptotic_optimal_rate} shows that we recover the optimal bound in Theorem \ref{thm:optimal_rate}, if the parameter $\lambda$ is set such that $\lambda = O(D^r),\, r\in ]0,2(\alpha-1)[$ in Algorithm \ref{algo:rna}.

If we further assume that we optimize a function with a Lipchitz-continuous Hessian, Proposition \ref{eq:bound_function_smooth_gradient} ensures that $e_i\leq D^2$. This means that we will recover asymptotically the optimal rate of convergence if $\lambda = O(D^r),\, r\in ]0,2[$. This improves the previous results in \citep{scieur2016regularized,scieur2017nonlinear} where $r\in ]0,\frac{3}{2}[$.
